Unleashing Hour-Scale Video Training for Long Video-Language Understanding

Recent long-form video-language understanding benchmarks have driven progress in video large multimodal models (Video-LMMs). However, the scarcity of well-annotated long videos has left the training of hour-long Video-LMMs underexplored. To close this gap, we present VideoMarathon, a large-scale hour-long video instruction-following dataset. This dataset includes around 9,700 hours of long videos sourced from diverse domains, ranging from 3 to 60 minutes per video. Specifically, it contains 3.3M high-quality QA pairs, spanning six fundamental topics: temporality, spatiality, object, action, scene, and event. Compared to existing video instruction datasets, VideoMarathon significantly extends training video durations up to 1 hour, and supports 22 diverse tasks requiring both short- and long-term video comprehension. Building on VideoMarathon, we propose Hour-LLaVA, a powerful and efficient Video-LMM for hour-scale video-language modeling. It enables hour-long video training and inference at 1-FPS sampling by leveraging a memory augmentation module, which adaptively integrates question-relevant and spatiotemporally informative semantics from the cached full video context. In our experiments, Hour-LLaVA achieves the best performance on multiple representative long video-language benchmarks, demonstrating the high quality of the VideoMarathon dataset and the superiority of the Hour-LLaVA model.

==> assets/figure/intro_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{assets/raw/intro_fig.pdf}
    \caption{\textbf{Comparison of video instruction-following datasets.} The x-axis denotes the video duration in minutes, while the y-axis indicates the number of QA pairs in millions. The proposed VideoMarathon fills the gap in long-video instruction tuning data (\textbf{3-60min}) and achieves a million-scale number of QA pairs.}
    \label{fig:intro_fig}
\end{figure}

==> assets/table/hourllava_comp.tex <==
\begin{wraptable}{r}{0.6\textwidth}
\centering
\vspace{-4mm}
\caption{\small \textbf{Comparison of video token compression methods}.
}
\vspace{-2mm}
\begin{adjustbox}{width=1\linewidth}\setlength\tabcolsep{3pt}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{TempCompass} & \textbf{LongVideoBench} & \textbf{LVBench} \\
\midrule
\rowcolor{orange!20} Hour-LLaVA & \textbf{59.7} & \textbf{54.0} & \textbf{40.6} \\
\midrule
Random  &  59.6 & 51.7 & 38.1 \\
Uniform~\cite{jiang2025token,xu2024slowfast} & 59.3 & 52.1 & 38.3 \\
Keyframe~\cite{shen2024longvu,tan2024koala} & 59.1 & 52.0 & 38.9 \\
User question-guided~\cite{di2025streaming,shen2024longvu} & 56.0 & 51.0 & 37.5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:method_comp}
\vspace{-2mm}
\end{wraptable}
